Searches for exclusive Higgs and $Z$ boson decays into $J/\psi\gamma$, $\psi(2S)\gamma$, and $\Upsilon(nS)\gamma$ at $\sqrt{s}=13$ TeV with the ATLAS detector

Searches for the exclusive decays of the Higgs and $Z$ bosons into a $J/\psi$, $\psi(2S)$, or $\Upsilon(nS)$ ($n=1,2,3$) meson and a photon are performed with a $pp$ collision data sample corresponding to an integrated luminosity of 36.1 fb$^{-1}$ collected at $\sqrt{s}=13$ TeV with the ATLAS detector at the CERN Large Hadron Collider. No significant excess of events is observed above the expected backgrounds, and 95% confidence-level upper limits on the branching fractions of the Higgs boson decays to $J/\psi\gamma$, $\psi(2S)\gamma$, and $\Upsilon(nS)\gamma$ of $3.5\times10^{-4}$, $2.0\times10^{-3}$, and $(4.9,5.9,5.7)\times10^{-4}$, respectively, are obtained assuming Standard Model production. The corresponding 95% confidence-level upper limits for the branching fractions of the $Z$ boson decays are $2.3\times10^{-6}$, $4.5\times10^{-6}$ and $(2.8,1.7,4.8)\times10^{-6}$, respectively.

==> auxiliary.tex <==
\subsection{Signal kinematic distributions: $\Jpsi\,\gamma$}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:dR_ph_muons_H}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/Signal_Dr_dimuons_H_Jpsi}}
\subfigure[\label{fig:dR_ph_muons_Z}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/Signal_Dr_dimuons_Z_Jpsi}}
\caption{$\Delta R_{\mu^+\mu^-}$ distributions for \subref{fig:dR_ph_muons_H} $H\to\Jpsi\gamma$ and \subref{fig:dR_ph_muons_Z} $Z\to\Jpsi\gamma$ simulated signal events. The solid lines denote the full event selection while the dashed lines show the events at generator level that fall within the detector acceptance (both muons are required to have $|\eta|<2.5$ and the photon within $|\eta|<2.37$ excluding the region $1.37<|\eta|<1.52$).}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:Pt_dimuons_H}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/Signal_Pt_dimuons_H_Jpsi}}
\subfigure[\label{fig:Pt_dimuons_Z}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/Signal_Pt_dimuons_Z_Jpsi}}
\caption{Generator level $\pt^{\mu^+\mu^-}$ distributions for \subref{fig:Pt_dimuons_H} $H\to\Jpsi\gamma$ and \subref{fig:Pt_dimuons_Z} $Z\to\Jpsi\gamma$ simulated signal events. The solid lines denote the full event selection while the dashed lines show the events at generator level that fall within the detector acceptance (both muons are required to have $|\eta|<2.5$ and the photon within $|\eta|<2.37$ excluding the region $1.37<|\eta|<1.52$).}
\end{figure}

\FloatBarrier
\subsection{Signal kinematic distributions: $\Upsilon(nS)\,\gamma$}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:dR_ph_muons_H_upsi}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/Signal_Dr_dimuons_H_Upsilon}}
\subfigure[\label{fig:dR_ph_muons_Z_upsi}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/Signal_Dr_dimuons_Z_Upsilon}}
\caption{$\Delta R_{\mu^{+}\mu^{-}}$ distributions for \subref{fig:dR_ph_muons_H_upsi} $H\to\Upsilon(nS)\gamma$ and \subref{fig:dR_ph_muons_Z_upsi} $Z\to\Upsilon(nS)\gamma$ simulated signal events. The solid lines denote the full event selection while the dashed lines show the events at generator level that fall within the detector acceptance (both muons are required to have $|\eta|<2.5$ and the photon within $|\eta|<2.37$ excluding the region $1.37<|\eta|<1.52$).}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:Pt_dimuons_H_upsi}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/Signal_Pt_dimuons_H_Upsilon}}
\subfigure[\label{fig:Pt_dimuons_Z_upsi}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/Signal_Pt_dimuons_Z_Upsilon}}
\caption{Generator level $\pt^{\mu^{+}\mu^{-}}$ distributions for \subref{fig:Pt_dimuons_H_upsi} $H\to\Upsilon(nS)\gamma$ and \subref{fig:Pt_dimuons_Z_upsi} $Z\to\Upsilon(nS)\gamma$ simulated signal events. The solid lines denote the full event selection while the dashed lines show the events at generator level that fall within the detector acceptance (both muons are required to have $|\eta|<2.5$ and the photon within $|\eta|<2.37$ excluding the region $1.37<|\eta|<1.52$).}
\end{figure}


\FloatBarrier
\subsection{Background control plots}

\begin{figure}[!h]
\centering
\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/h_Higgs_Mass_Jpsi_GR_1S_INC}
\caption{Plot of the three body mass of the $\psi(nS)\gamma$ system in the background generation region.\label{fig:Generation_Jpsi}}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:Generation_Upsi_B}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/h_Higgs_Mass_Upsilon_GR_B}}
\subfigure[\label{fig:Generation_Upsi_EC}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/h_Higgs_Mass_Upsilon_GR_EC}}
\caption{Plots of the three body mass of the $\Upsilon(nS)\gamma$ system in the background generation region, in the \subref{fig:Generation_Upsi_B} barrel and \subref{fig:Generation_Upsi_EC} endcap categories.\label{fig:Generation_Upsi}}
\end{figure}


\FloatBarrier
\subsection{Fit results in mass regions}

\begin{figure}[!h]
  \centering
  \subfigure[\label{fig:FitJpsi_ZBoson}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/JpsiFitReg_ZBoson}}
  \subfigure[\label{fig:FitJpsi_Higgs}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/JpsiFitReg_Higgs}}
\caption{The $m_\mumu$ distributions of the selected $\psi(nS)\gamma$ candidates within the three body invariant mass regions \subref{fig:FitJpsi_ZBoson} $86 < m_{\mumu\gamma} < 96$ GeV and \subref{fig:FitJpsi_Higgs} $120 < m_{\mumu\gamma} < 130$ GeV, along with the results of the maximum-likelihood fit with a background-only model. The Higgs and $Z$ boson contributions for the branching fraction values corresponding to the observed 95\% CL upper limits are also shown.\label{fig:FitJpsi2}}
\end{figure}

\begin{figure}[!h]
  \centering
  \subfigure[\label{fig:FitJpsi2_1S}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/JpsiFitReg_1S}}
  \subfigure[\label{fig:FitJpsi2_2S}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/JpsiFitReg_2S}}
\caption{The $m_{\mumu\gamma}$ distributions of the selected $\psi(nS)\gamma$ candidates within the dimuon invariant mass regions \subref{fig:FitJpsi2_1S} $2.9 < m_{\mumu} < 3.3$ GeV and \subref{fig:FitJpsi2_2S} $3.5 < m_{\mumu} < 3.9$ GeV, along with the results of the maximum-likelihood fit with a background-only model. The Higgs and $Z$ boson contributions for the branching fraction values corresponding to the observed 95\% CL upper limits are also shown.\label{fig:FitJpsi_nS}}
\end{figure}


\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_1S_ZBoson}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_1S_ZBoson}}
\subfigure[\label{fig:FitUpsi_EC_1S_ZBoson}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_1S_ZBoson}}
\caption{The $m_\mumu$ distributions of the selected $\Upsilon(nS)\gamma$ candidates within the three body invariant mass region $86 < m_{\mumu\gamma} < 96$ GeV in the \subref{fig:FitUpsi_B_1S_ZBoson} barrel and \subref{fig:FitUpsi_EC_1S_ZBoson} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $Z\to\Upsilon(1S)\gamma$ contribution for the branching fraction value corresponding to the observed 95\% CL upper limit is also shown.\label{fig:FitUpsi_1S_ZBoson}}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_2S_ZBoson}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_2S_ZBoson}}
\subfigure[\label{fig:FitUpsi_EC_2S_ZBoson}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_2S_ZBoson}}
\caption{The $m_\mumu$ distributions of the selected $\Upsilon(nS)\gamma$ candidates within the three body invariant mass region $86 < m_{\mumu\gamma} < 96$ GeV in the \subref{fig:FitUpsi_B_2S_ZBoson} barrel and \subref{fig:FitUpsi_EC_2S_ZBoson} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $Z\to\Upsilon(2S)\gamma$ contribution for the branching fraction value corresponding to the observed 95\% CL upper limit is also shown.\label{fig:FitUpsi_2S_ZBoson}}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_3S_ZBoson}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_3S_ZBoson}}
\subfigure[\label{fig:FitUpsi_EC_3S_ZBoson}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_3S_ZBoson}}
\caption{The $m_\mumu$ distributions of the selected $\Upsilon(nS)\gamma$ candidates within the three body invariant mass region $86 < m_{\mumu\gamma} < 96$ GeV in the \subref{fig:FitUpsi_B_3S_ZBoson} barrel and \subref{fig:FitUpsi_EC_3S_ZBoson} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $Z\to\Upsilon(3S)\gamma$ contribution for the branching fraction value corresponding to the observed 95\% CL upper limit is also shown.\label{fig:FitUpsi_3S_ZBoson}}
\end{figure}


\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_1S_Higgs}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_1S_Higgs}}
\subfigure[\label{fig:FitUpsi_EC_1S_Higgs}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_1S_Higgs}}
\caption{The $m_\mumu$ distributions of the selected $\Upsilon(nS)\gamma$ candidates within the three body invariant mass region $120 < m_{\mumu\gamma} < 130$ GeV in the \subref{fig:FitUpsi_B_1S_Higgs} barrel and \subref{fig:FitUpsi_EC_1S_Higgs} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $H\to\Upsilon(1S)\gamma$ contribution for the branching fraction value corresponding to the observed 95\% CL upper limit is also shown.\label{fig:FitUpsi_1S_Higgs}}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_2S_Higgs}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_2S_Higgs}}
\subfigure[\label{fig:FitUpsi_EC_2S_Higgs}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_2S_Higgs}}
\caption{The $m_\mumu$ distributions of the selected $\Upsilon(nS)\gamma$ candidates within the three body invariant mass region $120 < m_{\mumu\gamma} < 130$ GeV in the \subref{fig:FitUpsi_B_2S_Higgs} barrel and \subref{fig:FitUpsi_EC_2S_Higgs} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $H\to\Upsilon(2S)\gamma$ contribution for the branching fraction value corresponding to the observed 95\% CL upper limit is also shown.\label{fig:FitUpsi_2S_Higgs}}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_3S_Higgs}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_3S_Higgs}}
\subfigure[\label{fig:FitUpsi_EC_3S_Higgs}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_3S_Higgs}}
\caption{The $m_\mumu$ distributions of the selected $\Upsilon(nS)\gamma$ candidates within the three body invariant mass region $120 < m_{\mumu\gamma} < 130$ GeV in the \subref{fig:FitUpsi_B_3S_Higgs} barrel and \subref{fig:FitUpsi_EC_3S_Higgs} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $H\to\Upsilon(3S)\gamma$ contribution for the branching fraction value corresponding to the observed 95\% CL upper limit is also shown.\label{fig:FitUpsi_3S_Higgs}}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_1S}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_1S_1S}}
\subfigure[\label{fig:FitUpsi_EC_1S}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_1S_1S}}
\caption{The $m_{\mumu\gamma}$ distributions of the selected $\Upsilon(nS)\gamma$ candidates with a dimuon invariant mass within the region $9.0 < m_{\mumu} < 10.0$ GeV in the \subref{fig:FitUpsi_B_1S} barrel and \subref{fig:FitUpsi_EC_1S} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $H\to\Upsilon(1S)\gamma$ and $Z\to\Upsilon(1S)\gamma$ contributions for the branching fraction values corresponding to the observed 95\% CL upper limits are also shown.\label{fig:FitJpsi3_1S}}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_2S}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_2S_2S}}
\subfigure[\label{fig:FitUpsi_EC_2S}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_2S_2S}}
\caption{The $m_{\mumu\gamma}$ distributions of the selected $\Upsilon(nS)\gamma$ candidates with a dimuon invariant mass within the region $9.5 < m_{\mumu} < 10.5$ GeV in the \subref{fig:FitUpsi_B_1S} barrel and \subref{fig:FitUpsi_EC_1S} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $H\to\Upsilon(2S)\gamma$ and $Z\to\Upsilon(2S)\gamma$ contributions for the branching fraction values corresponding to the observed 95\% CL upper limits are also shown.\label{fig:FitJpsi3_2S}}
\end{figure}

\begin{figure}[!h]
\centering
\subfigure[\label{fig:FitUpsi_B_3S}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_B_3S_3S}}
\subfigure[\label{fig:FitUpsi_EC_3S}]{\includegraphics[width=0.45\textwidth]{figures/auxiliary_plots/UpsiFitReg_EC_3S_3S}}
\caption{The $m_{\mumu\gamma}$ distributions of the selected $\Upsilon(nS)\gamma$ candidates with a dimuon invariant mass within the region $10.0 < m_{\mumu} < 11.0$ GeV in the \subref{fig:FitUpsi_B_1S} barrel and \subref{fig:FitUpsi_EC_1S} endcap categories, along with the results of the maximum-likelihood fit with a background-only model. The $H\to\Upsilon(3S)\gamma$ and $Z\to\Upsilon(3S)\gamma$ contributions for the branching fraction values corresponding to the observed 95\% CL upper limits are also shown.\label{fig:FitJpsi_3S}}
\end{figure}


